Topic Modeling of Hierarchical Corpora

We study the problem of topic modeling in corpora whose documents are organized in a multi-level hierarchy. We explore a parametric approach to this problem, assuming that the number of topics is known or can be estimated by cross-validation. The models we consider can be viewed as special (finite-dimensional) instances of hierarchical Dirichlet processes (HDPs). For these models we show that there exists a simple variational approximation for probabilistic inference. The approximation relies on a previously unexploited inequality that handles the conditional dependence between Dirichlet latent variables in adjacent levels of the model's hierarchy. We compare our approach to existing implementations of nonparametric HDPs. On several benchmarks we find that our approach is faster than Gibbs sampling and able to learn more predictive models than existing variational methods. Finally, we demonstrate the large-scale viability of our approach on two newly available corpora from researchers in computer security---one with 350,000 documents and over 6,000 internal subcategories, the other with a five-level deep hierarchy.

==> corpora.tex <==
\section{Background on Corpora}
\label{app:background_on_corpora}

The Freelancer corpus collects seven years of job postings from Freelancer.com, one of the largest crowdsourcing sites on the Internet.  
The postings can be grouped by advertiser to form the three-level hierarchy shown in Fig.~\ref{figure:freelancer_hierarchy}.  
In this hierarchy, tiLDA models the advertisers as second-level interior nodes and the job postings as third-level leaf nodes.  

 The BlackHatWorld corpus collects over two years of postings from the ``BlackHatWorld'' Internet forum.  This data set was collected as part of a larger effort~\citep{Motoyama_Analysis_2011} to examine the social networks that develop in underground forums among distrustful parties.  The BlackHatWorld forum evolved to discuss abusive
% officially discouraged 
forms of Internet marketing, such as bulk emailing (spam).  The discussions are organized into the multi-level hierarchy shown in Fig.~\ref{figure:blackhatworld_hierarchy}.  We treat the threads in these subforums as documents for topic modeling.  (We do not consider individual posts within threads as documents because they are quite short.)
 
We preprocessed these two corpora in the same way, removing stopwords from a standard list~\citep{david_smart_2004}, discarding infrequent words that appeared in fewer than 6 documents,
and stemming the words that remain.  In both data sets, we also pruned ``barren" branches of the hierarchy: specifically, in the Freelancer corpus, we pruned advertisers with fewer than $20$ job postings, and in the BlackHatWorld corpus, we pruned subforums with fewer than $60$ threads.  


==> more_results.tex <==
 \section{Additional Results}

% Table~\ref{table:topics_freelancer} offers just a partial snapshot of the Freelancer corpus.  Others topics (not shown) describe legitimate forms of employment in Web site development, logo design, and app development.  We estimated the overall profile of job types on Freelancer.com by summing the topic proportions over all postings.  This sum suggests that roughly 30\% of all advertised jobs relate to some form of Web service abuse.  

The multi-level tiLDA models can also be used to analyze hierarchical corpora in ways that go beyond the discovery of global topics.  Recall that each tiLDA model yields topic proportions $\theta_t$ and a concentration parameter $\alpha_t$ for each category of the corpus.  We can analyze these proportions and parameters for further insights into hierarchical corpora.  In general, they provide a wealth of information beyond what can be discerned from (say) ordinary LDA.

\begin{table}[tb]
	\caption{Estimated ratio of number of buyers in job types on the Freelancer data set.}
	\label{table:buyer_ratio}
\begin{center} 
	\begin{tabular}{ll|ll} 
		\multicolumn{1}{l}{\bf  Type}  		&\multicolumn{1}{l}{\bf  Ratio}  		&\multicolumn{1}{l}{\bf Type}		&\multicolumn{1}{l}{\bf Ratio} 	\\ 
		\hline
		SEO				&18.47\%	&Affiliate Program	&3.21\% \\
		Captcha Solving	&2.68\%		&Account Creation	&1.42\% \\
		Bulk Emailing	&1.85\%		&OSN Linking		&2.12\% \\
		Ad Posting		&2.50\%		&Benign Jobs		&67.74\% \\
	\end{tabular} 
\end{center} 
\end{table}


Consider for example the Freelancer corpus.  In this corpus, the categories of tiLDA represent advertisers, and the topic proportions of these categories can be used to profile the types of jobs that advertisers are trying to crowdsource.  Summing these topic proportions over the corpus gives an estimate of the number of advertisers for each job type.  Table~\ref{table:buyer_ratio} shows the results of this estimate: it appears that nearly one-third of advertisers on Freelancer.com are commissioning abuse-related jobs, and of these jobs, the majority appear to involve some form of SEO.

We gain further insights by analyzing the concentration parameters of individual advertisers.  For example, the advertiser with the maximum concentration parameter ($\alpha_t=4065.00$) on Freelancer.com commissioned 34 projects, among which 32 have nearly the exact same description.  We also observe that advertisers with lower concentration parameters tend to be involved in a wider variety of projects.

On the BlackHatWorld corpus, the topic proportions and concentration parameters of categories generally reflect the titles of their associated subforums.  For example, the highest topic proportion (0.48) for ``Email Marketing" belongs to the subforum on `Email Marketing and Opt-In Lists,' and the highest topic proportion (0.59) for ``Blogging" belongs to the `Blogging' subforum.  The highest concentration parameter ($29.62$) belongs to the `Money, and Mo Money' subforum.  This is not surprising as this subforum itself has only four subforums as children, all of which are narrowly focused on specific revenue streams; see Fig.~\ref{figure:blackhatworld_hierarchy}.



